NIRANTAR: Continual Learning with New Languages and Domains on Real-world Speech Data

We introduce Nirantar, a comprehensive framework for evaluating continual learning (CL) in multilingual and multi-domain ASR. Designed to reflect real-world CL challenges, Nirantar leverages data collected incrementally across 22 languages and 208 districts in India through natural episodes. This enables evaluation across Language-Incremental (LIL), Domain-Incremental (DIL), and the novel Language-Incremental Domain-Incremental Learning (LIDIL) scenarios. Unlike prior work that relies on simulated episodes, Nirantar presents dynamic, non-uniform language and domain shifts, making it an ideal testbed for CL research. With 3250 hours of human-transcribed speech, including 1720 hours newly introduced in this work, our framework enables systematic benchmarking of CL methods. We evaluate existing approaches and demonstrate that no single method performs consistently well, underscoring the need for more robust CL strategies.

==> adapter_results.tex <==
\begingroup
\setlength{\tabcolsep}{4pt} % Default value: 6pt

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{lil-measures-with-adapters.png}
    \caption{Results on LIL scenario using different CL methods, including adapters.}
    \label{fig:lil-adapters}
    
\end{figure}
\endgroup

==> crosslingual_transfer.tex <==
\begingroup
\setlength{\tabcolsep}{4pt} % Default value: 6pt

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{lidil-measures.png}
    \caption{Comparison of different CL approaches for LIDIL scenario}
    \label{fig:lidil-cross-original}
    
    \includegraphics[width=\linewidth]{lidil-indo-aryan-measures.png}
    \caption{Comparison of different CL approaches for LIDIL scenario for IndoAryan language family splice.}
    \label{fig:lidil-cross-indoaryan}
    
    \includegraphics[width=\linewidth]{lidil-dravidian-measures.png}
    \caption{Comparison of different CL approaches for LIDIL scenario for Dravidian language family splice.}
    \label{fig:lidil-cross-dravidian}
\end{figure}
\endgroup

==> dataset_detailed_table.tex <==
% \begingroup
% \setlength{\tabcolsep}{4pt} % Default value: 6pt

% \begin{center}
% \small
% \begin{longtable}{ll|ccc|ccc}

% \caption{Table comparing different publicly available dataset and their usability in different CL scenarios}
% \label{tab:dataset_detailed_table} \\

% \toprule \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Language} \\ \textbf{Code}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Domain/}\\ \textbf{District}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Train} \\ \textbf{(hours)}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Test} \\ \textbf{(minutes)}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{WER} \\ \textbf{(on Test)}\end{tabular}} & \multicolumn{3}{c}{\textbf{Episodic presence}} \\
% \cmidrule{6-8}
%  &  &  & & & \textbf{LIL} & \textbf{DIL} & \textbf{LIDIL} \\
% \midrule
% \endfirsthead

% % \multicolumn{8}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
% \toprule \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Language} \\ \textbf{Code}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Domain/}\\ \textbf{District}\end{tabular}} & \multicolumn{1}{l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Train} \\ \textbf{(hours)}\end{tabular}}} & \multicolumn{1}{l}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Test} \\ \textbf{(minutes)}\end{tabular}}} & \multicolumn{1}{l}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{WER} \\ \textbf{(on Test)}\end{tabular}}} & \multicolumn{3}{c}{\textbf{Episodic presence}} \\
% \cmidrule{6-8}
%  &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{LIL} & \textbf{DIL} & \textbf{LIDIL} \\
% \midrule
% \endhead

% \midrule \multicolumn{8}{r}{{Continued on next page}} \\ \bottomrule
% \endfoot

% \hline \hline
% \endlastfoot

% as & Barpeta & 12 & 15.1 & 22.3\% & episode0 & episode0 & episode0 \\
% as & Biswanath & 18 & 15.1 & 16.3\% & episode0 & episode0 & episode10 \\
% as & Charaideo & 7.7 & 15.0 & 18.9\% & episode0 & episode0 & episode9 \\
% as & Darrang & 14.3 & 15.1 & 24.4\% & episode0 & episode3 & episode6 \\
% as & Dhemaji & 19.4 & 15.1 & 17.6\% & episode0 & episode8 & episode10 \\
% as & Dibrugarh & 17.6 & 15.0 & 19.1\% & episode0 & episode2 & episode10 \\
% as & Kamrup Metropolitan & 21.8 & 15.0 & 21.8\% & episode0 & episode11 & episode0 \\
% as & Lakhimpur & 38.6 & 15.0 & 22.1\% & episode0 & episode11 & episode0 \\
% as & Morigaon & 20.3 & 15.2 & 25.6\% & episode0 & episode0 & episode0 \\
% as & Nagaon & 18.7 & 15.1 & 23.3\% & episode0 & episode0 & episode0 \\
% as & Nalbari & 24.9 & 15.0 & 25.5\% & episode0 & episode4 & episode0 \\
% as & Sivasagar & 0.6 & 5.8 & 18.5\% & episode0 & episode0 & episode0 \\
% as & Sonitpur & 17.6 & 15.1 & 17.6\% & episode0 & episode0 & episode3 \\
% as & Tinsukia & 5.3 & 15.0 & 18.2\% & episode0 & episode6 & episode6 \\
% bn & Jalpaiguri & 0.8 & 15.1 & 18.8\% & episode0 & episode11 & episode7 \\
% bn & Jhargram & 28.9 & 15.1 & 15.2\% & episode0 & episode0 & episode11 \\
% bn & Nadia & 24.1 & 15.0 & 17.7\% & episode0 & episode11 & episode0 \\
% bn & North 24 Parganas & 2.9 & 15.1 & 13.5\% & episode0 & episode9 & episode0 \\
% bn & Paschim Bardhaman & 31.7 & 15.0 & 15.7\% & episode0 & episode11 & episode6 \\
% bn & Paschim Medinipur & 29.8 & 15.0 & 16.6\% & episode0 & episode7 & episode0 \\
% bn & Purba Bardhaman & 24.7 & 15.0 & 17.9\% & episode0 & episode0 & episode0 \\
% bn & Purba Medinipur & 23.2 & 15.0 & 17.7\% & episode0 & episode0 & episode5 \\
% bn & Purulia & 19.5 & 15.2 & 16.6\% & episode0 & episode0 & episode7 \\
% bn & South 24 Parganas & 18.7 & 15.0 & 17.8\% & episode0 & episode0 & episode4 \\
% brx & Baksa & 51.3 & 15.1 & 26.3\% & episode0 & episode9 & episode0 \\
% brx & Chirang & 106.2 & 15.1 & 28.2\% & episode0 & episode0 & episode11 \\
% brx & Kokrajhar & 81.3 & 15.1 & 29.0\% & episode0 & episode5 & episode0 \\
% brx & Udalguri & 46.2 & 15.0 & 30.8\% & episode0 & episode0 & episode6 \\
% hi & Darbhanga & 3.4 & 15.1 & 13.5\% & episode0 & episode0 & episode0 \\
% hi & Balaghat & 7.6 & 15.1 & 16.7\% & episode0 & episode0 & episode0 \\
% hi & Bhopal & 26.9 & 15.2 & 12.6\% & episode0 & episode0 & episode7 \\
% hi & Gwalior & 2.2 & 15.0 & 15.2\% & episode0 & episode3 & episode5 \\
% hi & Jabalpur & 2.2 & 15.2 & 16.9\% & episode0 & episode0 & episode11 \\
% hi & Katni & 1.6 & 15.0 & 15.2\% & episode0 & episode0 & episode10 \\
% hi & Jaipur & 27.3 & 15.1 & 16.3\% & episode0 & episode0 & episode1 \\
% hi & Jodhpur & 25.2 & 15.1 & 17.4\% & episode0 & episode4 & episode0 \\
% hi & Karauli & 10.2 & 15.1 & 16.4\% & episode0 & episode8 & episode6 \\
% hi & Bhadohi & 2.2 & 15.1 & 17.0\% & episode0 & episode11 & episode0 \\
% hi & Mirzapur & 4.9 & 15.0 & 18.0\% & episode0 & episode11 & episode0 \\
% hi & Sonbhadra & 20.7 & 15.1 & 16.8\% & episode0 & episode8 & episode0 \\
% mai & Darbhanga & 34.6 & 15.0 & 30.7\% & episode0 & episode11 & episode2 \\
% mai & Begusarai & 0.3 & 5.5 & 32.5\% & episode0 & episode11 & episode4 \\
% mai & Madhubani & 33.3 & 15.0 & 32.0\% & episode0 & episode2 & episode0 \\
% mai & Muzaffarpur & 26.8 & 15.1 & 32.7\% & episode0 & episode0 & episode5 \\
% mai & Purnia & 40.9 & 15.1 & 41.0\% & episode0 & episode0 & episode0 \\
% mai & Saharsa & 26.8 & 15.2 & 32.3\% & episode0 & episode4 & episode4 \\
% mai & Samastipur & 7.3 & 15.0 & 40.4\% & episode0 & episode11 & episode0 \\
% mai & Sitamarhi & 32.7 & 15.4 & 38.8\% & episode0 & episode0 & episode8 \\
% mai & Supaul & 39.9 & 15.0 & 35.7\% & episode0 & episode0 & episode0 \\
% ml & Ernakulam & 0.1 & 11.7 & 32.3\% & episode0 & episode10 & episode10 \\
% ml & Kannur & 14.4 & 15.2 & 41.6\% & episode0 & episode0 & episode0 \\
% ml & Kasaragod & 11 & 15.0 & 36.4\% & episode0 & episode0 & episode6 \\
% ml & Kottayam & 12.4 & 15.1 & 39.4\% & episode0 & episode0 & episode0 \\
% ml & Kozhikode & 40.1 & 15.1 & 37.4\% & episode0 & episode1 & episode0 \\
% ml & Malappuram & 1.2 & 15.1 & 34.2\% & episode0 & episode2 & episode1 \\
% ml & Palakkad & 45.5 & 15.1 & 39.3\% & episode0 & episode0 & episode10 \\
% ml & Thiruvananthapuram & 6.9 & 15.0 & 37.8\% & episode0 & episode0 & episode6 \\
% ml & Thrissur & 1.8 & 3.9 & 39.6\% & episode0 & episode3 & episode0 \\
% ml & Wayanad & 32.5 & 15.2 & 44.8\% & episode0 & episode9 & episode0 \\
% ne & Jalpaiguri & 22.5 & 15.2 & 20.6\% & episode0 & episode0 & episode0 \\
% ne & Alipurduar & 1.3 & 15.1 & 25.8\% & episode0 & episode2 & episode0 \\
% ne & Darjeeling & 109.8 & 15.1 & 17.1\% & episode0 & episode0 & episode9 \\
% ne & Kalimpong & 113.3 & 15.0 & 17.0\% & episode0 & episode1 & episode3 \\
% pa & Fatehgarh Sahib & 27.8 & 15.0 & 15.2\% & episode0 & episode8 & episode0 \\
% pa & Mohali & 34.5 & 15.0 & 11.7\% & episode0 & episode0 & episode0 \\
% pa & Patiala & 1.5 & 15.1 & 17.0\% & episode0 & episode0 & episode11 \\
% pa & Rupnagar & 30.5 & 15.0 & 13.5\% & episode0 & episode7 & episode6 \\
% pa & Shaheed Bhagat Singh Nagar & 27.5 & 15.0 & 12.3\% & episode0 & episode7 & episode9 \\
% sat & Jhargram & 22 & 15.1 & 29.2\% & episode0 & episode11 & episode0 \\
% sat & Paschim Bardhaman & 26.4 & 15.1 & 31.4\% & episode0 & episode11 & episode10 \\
% sat & Purba Bardhaman & 21.7 & 15.1 & 35.3\% & episode0 & episode0 & episode0 \\
% sat & Purulia & 6.3 & 15.0 & 46.7\% & episode0 & episode11 & episode1 \\
% sat & Bankura & 33.8 & 15.1 & 34.3\% & episode0 & episode0 & episode7 \\
% sat & Birbhum & 45.7 & 15.0 & 40.3\% & episode0 & episode0 & episode0 \\
% sat & Malda & 1.4 & 15.0 & 40.4\% & episode0 & episode0 & episode6 \\
% sat & Uttar Dinajpur & 2.9 & 15.0 & 47.6\% & episode0 & episode11 & episode0 \\
% ta & Ariyalur & 4.4 & 15.1 & 29.0\% & episode0 & episode3 & episode11 \\
% ta & Coimbatore & 12.9 & 15.1 & 36.3\% & episode0 & episode11 & episode8 \\
% ta & Cuddalore & 11.7 & 15.0 & 31.4\% & episode0 & episode1 & episode0 \\
% ta & Dharmapuri & 12.1 & 15.0 & 34.7\% & episode0 & episode0 & episode6 \\
% ta & Erode & 15.3 & 15.1 & 33.9\% & episode0 & episode0 & episode0 \\
% ta & Kallakurichi & 16 & 15.0 & 32.0\% & episode0 & episode0 & episode7 \\
% ta & Krishnagiri & 13.8 & 15.0 & 32.6\% & episode0 & episode0 & episode0 \\
% ta & Mayiladuthurai & 32.2 & 15.1 & 34.9\% & episode0 & episode11 & episode2 \\
% ta & Nagapattinam & 20.4 & 15.1 & 37.1\% & episode0 & episode0 & episode0 \\
% ta & Namakkal & 21 & 15.1 & 37.1\% & episode0 & episode0 & episode0 \\
% ta & Perambalur & 2.6 & 15.1 & 37.1\% & episode0 & episode10 & episode4 \\
% ta & Pudukkottai & 6 & 15.1 & 26.4\% & episode0 & episode4 & episode0 \\
% ta & Salem & 10.8 & 15.0 & 33.7\% & episode0 & episode0 & episode6 \\
% ta & Sivaganga & 15.1 & 15.1 & 35.2\% & episode0 & episode8 & episode0 \\
% ta & Thanjavur & 1.3 & 15.0 & 36.5\% & episode0 & episode11 & episode0 \\
% ta & Tiruchirappalli & 3.1 & 15.1 & 38.4\% & episode0 & episode5 & episode11 \\
% ta & Tiruppur & 11.6 & 15.0 & 35.9\% & episode0 & episode0 & episode11 \\
% ta & Tiruvarur & 16.6 & 15.1 & 29.9\% & episode0 & episode10 & episode11 \\
% ta & Viluppuram & 5.8 & 15.1 & 27.7\% & episode0 & episode0 & episode0 \\
% te & Anakapalli & 1.1 & 15.3 & 20.0\% & episode0 & episode11 & episode10 \\
% te & Chittoor & 19.1 & 15.1 & 26.6\% & episode0 & episode0 & episode0 \\
% te & East Godavari & 14.9 & 15.1 & 28.1\% & episode0 & episode11 & episode5 \\
% te & Eluru & 10.6 & 15.1 & 21.4\% & episode0 & episode0 & episode0 \\
% te & Guntur & 8.3 & 15.1 & 20.7\% & episode0 & episode1 & episode4 \\
% te & Kakinada & 15.9 & 15.0 & 29.8\% & episode0 & episode4 & episode0 \\
% te & Konaseema & 12.8 & 15.0 & 16.9\% & episode0 & episode6 & episode0 \\
% te & Krishna & 2.1 & 3.2 & 23.1\% & episode0 & episode0 & episode0 \\
% te & N T Rama Rao & 4.3 & 15.3 & 27.8\% & episode0 & episode3 & episode10 \\
% te & Nellore & 5.6 & 15.1 & 34.3\% & episode0 & episode2 & episode7 \\
% te & Palnadu & 8.2 & 15.1 & 21.3\% & episode0 & episode0 & episode0 \\
% te & Sri Balaji & 18.7 & 15.1 & 32.0\% & episode0 & episode4 & episode0 \\
% te & Srikakulam & 10.8 & 15.0 & 29.6\% & episode0 & episode0 & episode5 \\
% te & Visakhapatnam & 2.3 & 15.1 & 29.8\% & episode0 & episode0 & episode0 \\
% te & Vizianagaram & 9.9 & 15.0 & 30.3\% & episode0 & episode4 & episode3 \\
% te & West Godavari & 4.7 & 15.2 & 24.7\% & episode0 & episode9 & episode4 \\
% te & Hyderabad & 16.7 & 15.0 & 31.3\% & episode0 & episode0 & episode4 \\
% te & Karimnagar & 0 & 1.6 & 7.8\% & episode0 & episode8 & episode0 \\
% te & Mahbubnagar & 1.1 & 15.2 & 21.4\% & episode0 & episode3 & episode3 \\
% te & Mancherial & 4.5 & 15.2 & 30.1\% & episode0 & episode0 & episode8 \\
% te & Medchal & 4.3 & 15.1 & 27.0\% & episode0 & episode0 & episode7 \\
% te & Nalgonda & 7.5 & 15.1 & 29.8\% & episode0 & episode0 & episode0 \\
% te & Nirmal & 2.1 & 15.1 & 29.0\% & episode0 & episode3 & episode0 \\
% te & Ranga Reddy & 12.9 & 15.1 & 32.0\% & episode0 & episode11 & episode9 \\
% te & Sangareddy & 4.1 & 15.0 & 24.0\% & episode0 & episode0 & episode0 \\
% te & Vikarabad & 7.1 & 15.1 & 26.6\% & episode0 & episode0 & episode0 \\
% te & Yadadri Bhuvanagiri & 2.7 & 15.0 & 19.1\% & episode0 & episode0 & episode6 \\
% doi & Jammu & 12.2 & 15.1 & 30.4\% & episode1 & episode3 & episode2 \\
% doi & Kathua & 0.3 & 13.4 & 17.9\% & episode1 & episode7 & episode7 \\
% doi & Reasi & 55.1 & 15.2 & 30.1\% & episode1 & episode0 & episode11 \\
% doi & Samba & 0.8 & 4.9 & 22.4\% & episode1 & episode0 & episode7 \\
% doi & Udhampur & 45 & 15.0 & 35.6\% & episode1 & episode1 & episode2 \\
% sa & Chittoor & 3.9 & 15.1 & 19.6\% & episode10 & episode11 & episode3 \\
% sa & Bagalkot & 2 & 15.0 & 22.9\% & episode10 & episode0 & episode10 \\
% sa & Bangalore Rural & 0.6 & 15.1 & 21.4\% & episode10 & episode10 & episode11 \\
% sa & Bangalore Urban & 6.1 & 15.1 & 20.8\% & episode10 & episode11 & episode5 \\
% sa & Chikkamagaluru & 2.6 & 15.0 & 23.2\% & episode10 & episode0 & episode2 \\
% sa & Dakshina Kannada & 12.2 & 15.1 & 21.9\% & episode10 & episode0 & episode3 \\
% sa & Mysore & 3.8 & 15.0 & 17.3\% & episode10 & episode11 & episode8 \\
% sa & Shimoga & 4.3 & 15.1 & 20.3\% & episode10 & episode0 & episode1 \\
% sa & Udupi & 8.3 & 15.3 & 23.5\% & episode10 & episode0 & episode9 \\
% sa & Uttara Kannada & 11.4 & 15.1 & 22.3\% & episode10 & episode0 & episode3 \\
% sa & Nagpur & 0.6 & 15.1 & 17.4\% & episode10 & episode11 & episode9 \\
% sa & Jaipur & 2.6 & 15.2 & 24.7\% & episode10 & episode11 & episode2 \\
% sa & Coimbatore & 1.6 & 6.3 & 34.0\% & episode10 & episode0 & episode1 \\
% sa & Chennai & 3.3 & 15.1 & 24.0\% & episode10 & episode9 & episode5 \\
% sa & Hyderabad & 1.5 & 15.0 & 21.5\% & episode10 & episode11 & episode6 \\
% sa & Ranga Reddy & 0 & 15.0 & 21.7\% & episode10 & episode0 & episode5 \\
% sd & South Delhi & 0.1 & 2.0 & 21.6\% & episode11 & episode0 & episode5 \\
% sd & Surat & 2 & 15.0 & 20.0\% & episode11 & episode2 & episode3 \\
% sd & Mumbai Suburban & 3.5 & 15.0 & 20.8\% & episode11 & episode0 & episode7 \\
% sd & Thane & 20.5 & 15.1 & 23.2\% & episode11 & episode2 & episode1 \\
% ks & Anantnag & 11.2 & 15.1 & 43.5\% & episode2 & episode0 & episode1 \\
% ks & Bandipora & 3.7 & 15.2 & 30.8\% & episode2 & episode0 & episode2 \\
% ks & Baramulla & 11 & 15.1 & 45.8\% & episode2 & episode0 & episode7 \\
% ks & Budgam & 7.7 & 15.0 & 38.7\% & episode2 & episode0 & episode11 \\
% ks & Ganderbal & 16.5 & 15.1 & 34.8\% & episode2 & episode0 & episode10 \\
% ks & Kulgam & 16.2 & 15.0 & 45.6\% & episode2 & episode7 & episode1 \\
% ks & Kupwara & 11.8 & 15.1 & 42.7\% & episode2 & episode6 & episode11 \\
% ks & Pulwama & 2.5 & 15.2 & 36.4\% & episode2 & episode1 & episode1 \\
% ks & Shopian & 19.6 & 15.1 & 37.7\% & episode2 & episode9 & episode11 \\
% ks & Srinagar & 3.2 & 15.0 & 41.0\% & episode2 & episode2 & episode4 \\
% gu & Ahmedabad & 4.8 & 15.2 & 14.6\% & episode3 & episode5 & episode9 \\
% gu & Aravalli & 2.6 & 15.0 & 24.5\% & episode3 & episode0 & episode11 \\
% gu & Mehsana & 4.8 & 15.0 & 16.7\% & episode3 & episode0 & episode6 \\
% gu & Morbi & 6.9 & 15.2 & 20.4\% & episode3 & episode4 & episode7 \\
% ur & South Delhi & 12.4 & 15.0 & 13.1\% & episode4 & episode11 & episode6 \\
% ur & Central Delhi & 17 & 15.2 & 15.9\% & episode4 & episode0 & episode10 \\
% ur & Nashik & 14.1 & 15.0 & 13.6\% & episode4 & episode0 & episode10 \\
% ur & Hyderabad & 12.1 & 15.1 & 15.3\% & episode4 & episode11 & episode7 \\
% ur & Aligarh & 16.6 & 15.1 & 13.3\% & episode4 & episode0 & episode7 \\
% ur & Gautam Buddha Nagar & 18.5 & 15.2 & 13.4\% & episode4 & episode8 & episode4 \\
% ur & Ghaziabad & 2.6 & 14.3 & 19.2\% & episode4 & episode0 & episode10 \\
% ur & Lucknow & 18.2 & 15.1 & 14.1\% & episode4 & episode0 & episode3 \\
% ur & Mau & 3.6 & 15.1 & 13.8\% & episode4 & episode5 & episode8 \\
% ur & Shahjahanpur & 5.8 & 15.1 & 10.8\% & episode4 & episode6 & episode11 \\
% kok & Bardez & 33.1 & 15.1 & 32.3\% & episode5 & episode0 & episode11 \\
% kok & Canacona & 46.2 & 15.0 & 32.7\% & episode5 & episode0 & episode9 \\
% kok & Tiswadi & 20.3 & 15.1 & 27.9\% & episode5 & episode7 & episode10 \\
% or & Bhadrak & 2.2 & 15.0 & 18.6\% & episode6 & episode0 & episode11 \\
% or & Boudh & 12.5 & 15.0 & 28.8\% & episode6 & episode11 & episode1 \\
% or & Cuttack & 0 & 0.7 & 37.5\% & episode6 & episode3 & episode8 \\
% or & Dhenkanal & 20.8 & 15.3 & 23.7\% & episode6 & episode0 & episode10 \\
% or & Jajpur & 15.3 & 15.1 & 22.0\% & episode6 & episode0 & episode8 \\
% or & Kalahandi & 0 & 1.2 & 42.9\% & episode6 & episode11 & episode1 \\
% or & Kandhamal & 21.6 & 15.1 & 21.3\% & episode6 & episode0 & episode9 \\
% or & Khordha & 26.4 & 15.1 & 21.0\% & episode6 & episode11 & episode8 \\
% or & Nayagarh & 22.3 & 15.0 & 22.9\% & episode6 & episode2 & episode9 \\
% mr & Nagpur & 15 & 15.0 & 18.9\% & episode7 & episode0 & episode11 \\
% mr & Thane & 4.3 & 15.1 & 16.5\% & episode7 & episode2 & episode10 \\
% mr & Akola & 24.9 & 15.2 & 17.1\% & episode7 & episode10 & episode9 \\
% mr & Amravati & 16.2 & 15.1 & 18.7\% & episode7 & episode11 & episode1 \\
% mr & Buldhana & 18.9 & 15.0 & 17.6\% & episode7 & episode0 & episode9 \\
% mr & Raigad & 0.6 & 6.8 & 18.0\% & episode7 & episode0 & episode5 \\
% mr & Solapur & 1.4 & 2.1 & 16.8\% & episode7 & episode0 & episode4 \\
% mr & Wardha & 2.5 & 15.1 & 16.4\% & episode7 & episode1 & episode3 \\
% mr & Washim & 7.5 & 15.1 & 22.3\% & episode7 & episode0 & episode9 \\
% mr & Yavatmal & 23.9 & 15.1 & 16.2\% & episode7 & episode2 & episode9 \\
% kn & Bangalore Rural & 5.7 & 15.0 & 34.2\% & episode8 & episode10 & episode2 \\
% kn & Bangalore Urban & 4 & 15.1 & 30.4\% & episode8 & episode0 & episode8 \\
% kn & Mysore & 1.2 & 2.1 & 43.6\% & episode8 & episode0 & episode5 \\
% kn & Shimoga & 17.6 & 15.0 & 22.2\% & episode8 & episode11 & episode4 \\
% kn & Udupi & 1.6 & 13.4 & 29.2\% & episode8 & episode0 & episode2 \\
% kn & Bidar & 8.1 & 15.0 & 43.6\% & episode8 & episode1 & episode4 \\
% kn & Chamarajanagar & 1.5 & 1.3 & 29.2\% & episode8 & episode0 & episode3 \\
% kn & Chikkaballapur & 8.3 & 15.1 & 22.2\% & episode8 & episode8 & episode6 \\
% kn & Chitradurga & 10.9 & 15.0 & 29.1\% & episode8 & episode5 & episode11 \\
% kn & Davanagere & 8.9 & 15.1 & 30.6\% & episode8 & episode0 & episode10 \\
% kn & Kolar & 14 & 15.2 & 23.8\% & episode8 & episode0 & episode8 \\
% kn & Tumkur & 11.4 & 15.0 & 26.9\% & episode8 & episode1 & episode9 \\
% mni & Imphal West & 18.6 & 15.1 & 21.6\% & episode9 & episode4 & episode7 \\
% mni & Kakching & 3.7 & 15.0 & 37.3\% & episode9 & episode0 & episode10 \\
% mni & Thoubal & 18.3 & 15.1 & 21.8\% & episode9 & episode11 & episode4 
% \end{longtable}
% \end{center}

% \endgroup

==> domain_vocab_evolution.tex <==
\begingroup
\setlength{\tabcolsep}{4pt} % Default value: 6pt

\begin{figure}[!h]
    
    \centering  
    \includegraphics[width=0.5\linewidth]{cumulative_domain.png}
    \caption{Figure showing the cumulative improvement of domains across episodes.}
    \label{fig:cumulative_domain}
\end{figure}
\begin{figure}[!h]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{cumulative_vocab_train.png}
        \caption{Training set.}
        \label{fig:cumulative_vocab_train}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\linewidth]{cumulative_vocab_test.png}
        \caption{Test set.}
        \label{fig:cumulative_vocab_test}
    \end{subfigure}
    \caption{Comparison of cumulative vocabulary improvement across episodes for training and test sets.}
    \label{fig:cumulative_vocab}
\end{figure}
\endgroup

==> multiple_task_order.tex <==
\begingroup
\setlength{\tabcolsep}{4pt} % Default value: 6pt

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{lidil-measures.png}
    \caption{Random Order 1 for LIDIL Scenario.}
    \label{fig:lidil-original}
    
    \includegraphics[width=\linewidth]{lidil-measures-perm-1.png}
    \caption{Random Order 2 for LIDIL Scenario.}
    \label{fig:lidil-perm1}
    
    \includegraphics[width=\linewidth]{lidil-measures-perm-2.png}
    \caption{Random Order 3 for LIDIL Scenario}
    \label{fig:lidil-perm2}
\end{figure}
\endgroup
